ARMOR: A Model-based Framework for Improving Arbitrary Baseline Policies with Offline Data

We propose a new model-based offline RL framework, called Adversarial Models for Offline Reinforcement Learning (ARMOR), which can robustly learn policies to improve upon an arbitrary baseline policy regardless of data coverage. Based on the concept of relative pessimism, ARMOR is designed to optimize for the worst-case relative performance when facing uncertainty. In theory, we prove that the learned policy of ARMOR never degrades the performance of the baseline policy with any admissible hyperparameter, and can learn to compete with the best policy within data coverage when the hyperparameter is well tuned, and the baseline policy is supported by the data. Such a robust policy improvement property makes ARMOR especially suitable for building real-world learning systems, because in practice ensuring no performance degradation is imperative before considering any benefit learning can bring.

==> fixed_point.tex <==
Given \algo's ability to improve over an arbitrary policy, the following questions naturally arise:
\begin{center}\it 
Can \algo nontrivially improve the output policy of other algorithms (e.g., such as those based on \emph{absolute pessimism} \citep{xie2021bellman}), including itself?
\end{center}
Note that we can always output $\piref$ itself to guarantee improvement, but such improvement is trivial as the worst-case improvement is $0$. By ``nontrivially'' we mean a non-zero worst-case improvement; otherwise, the statement would be meaningless. If the statement were true, we would be able to repeatedly run \algo to continuously improve over its own output and hopefully obtain better performance with more iterations. 

Unfortunately, the answer is negative. Not only \algo cannot improve over itself, but it also cannot improve over a variety of algorithms. In fact, the optimal policy of an \textit{arbitrary} model in the version space is unimprovable (see Corollary~\ref{th:fixed-point examples})! Our discussion reveals some interesting observations (e.g., how equivalent performance metrics for online RL can behave very differently in the offline setting) and their implications (e.g., how we should choose $\piref$ for \algo). Despite their simplicity, we feel that many in the offline RL community are not actively aware of these facts (and the unawareness has led to some confusion), which we hope to clarify with our discussion below.

\paragraph{Setup} We consider the setup where the decision maker is given a version space $\Mcal_\alpha$ that contains the true model ($M^\star \in \Mcal_\alpha$), and need to choose a policy $\pi \in\Pi$ based on $\Mcal_\alpha$. We use the same notation $\Mcal_\alpha$ as in the main paper, but emphasize that it does not have to be constructed as in \eqref{eq:v_space} and \eqref{eq:def_loss}. In fact, for the purpose of this discussion, the data distribution, the sample size, the data randomness, and the estimation procedure for constructing $\Mcal_\alpha$ are \textbf{all irrelevant}, as our focus here is how decisions should be made with a given $\Mcal_\alpha$. This makes our setup very generic and the conclusions widely applicable.

To facilitate discussion, we define the \textit{fixed point} of \algo's relative pessimism step:
\begin{definition} \label{def:fixed_point}
Consider \eqref{eq:def_pihat} as an operator that maps an arbitrary policy $\piref$ to $\pihat$. A fixed point of this \emph{relative pessimism} operator is, therefore, any policy $\pi \in \Pi$ such that
$$
\pi \in \argmax_{\pi' \in \Pi} \min_{M \in \Mcal_\alpha} J_M(\pi') - J_M(\pi).
$$
\end{definition}
Given the definition, relative pessimism cannot improve over a policy if it is already a fixed point. Below we show a sufficient and necessary condition for being a fixed point, which further leads to a number of concrete examples. 


\begin{lemma}[Fixed-point Lemma] \label{lm:fixed-point lm of mb-atac}
For any $\Mcal \subseteq \Mcal_\alpha$ and any $\psi:\Mcal\to\mathbb{R}$, consider the policy
\begin{align} \label{eq:candidate fixed-point policies}
    \pi \in \argmax_{\pi'\in\Pi} \min_{M\in\Mcal} J_M(\pi') + \psi(M)
\end{align}
Then $\pi$ is a fixed point in Definition~\ref{def:fixed_point}.
Conversely, for any fixed point $\pi$ in \cref{def:fixed_point}, there is a $\psi:\Mcal\to\mathbb{R}$ such that $\pi$ is a solution to \eqref{eq:candidate fixed-point policies}.
\end{lemma}
\begin{proof}
We prove the result by contradiction.
First notice $\min_{M\in\Mcal} J_M(\pi') - J_M(\pi') = 0$.
Suppose there is $\overline{\pi} \in \Pi$ such that $\min_{M\in\Mcal_\alpha} J_M(\bar{\pi}) - J_M(\pi') >0$, which implies that $J_M(\bar{\pi}) >J_M(\pi') $, $\forall M \in \Mcal_\alpha$.
%Let $\overline{M} = \argmin_{M\in\Mcal} J_M(\bar{\pi}) - J_M(\pi')$. This would imply that 
Since $\Mcal \subseteq \Mcal_\alpha$, we have 
\begin{align*}
    \min_{M\in\Mcal} J_M(\bar{\pi})  + \psi(M) 
    &>  \min_{M\in\Mcal}  J_M(\pi')  + \psi(M) =  \max_{\pi\in\Pi}\min_{M\in\Mcal}  J_M(\pi)  + \psi(M)
\end{align*}
which is a contradiction of the maximin optimality. Thus $\max_{\pi\in\Pi} \min_{M\in\Mcal_\alpha} J_M(\bar{\pi}) - J_M(\pi') = 0 $, which means $\pi'$ is a solution.

For the converse statement, suppose $\pi$ is a fixed point. We can just let $\psi(M) = -J_M(\pi)$. Then this pair of $\pi$ and $\psi$ by definition of the fixed point satisfies \eqref{eq:candidate fixed-point policies}.
\end{proof}

With this lemma, we can show a number of concrete examples (some of which may be surprising) that are fixed points and thus unimprovable:


%We can view that function $\psi$ as a regularization term on the MDP player. We can use \eqref{eq:candidate fixed-point policies} to instantiate different algorithms and \cref{lm:fixed-point lm of mb-atac} shows that the solution to these algorithms are fixed points of relative pessimism. In particular, this result implies that we cannot iterate relative pessimism forever; it would converge in one iteration.
\begin{corollary} \label{th:fixed-point examples}
The following are fixed points of relative pessimism (Definition~\ref{def:fixed_point}):
\begin{enumerate}
    \item  Absolute-pessimism policy, i.e., $\psi(M) = 0 $.
    \item Relative-pessimism policy for any reference policy, i.e., $\psi(M) = - J_M(\piref)$. 
    \item Regret-minimization policy, i.e., $\psi(M) = -J_M(\pi_M^*)$, where $\pi_M^* \in \argmax_{\pi\in\Pi} J_M(\pi)$ is an optimal policy for $M$.
    \item Optimal policy of an \emph{arbitrary} model $M \in \Mcal_\alpha$, $\pi_M^*$, i.e., $\Mcal = \{M\}$. 
    This would include the optimistic policy, that is, $\argmax_{\pi\in\Pi, M\in\Mcal_\alpha} J_M(\pi)$
    %\nan{UCB $\Rightarrow$ optimistic? also, define and add citations?}
\end{enumerate}
\end{corollary}

We now have a discussion about absolute pessimism (\#1) vs.~regret minimization (\#3), and then extend the lesson to the more general setting. 

\paragraph{Return maximization and regret minimization are \textit{different} in offine RL} We first note that these four examples generally produce different policies, even though some of them optimize for objectives that are traditionally viewed as equivalent in online RL (that is, if we ignore the ``worst-case over $\Mcal_\alpha$'' part of the definition), e.g., absolute pessimism optimizes for $J_M(\pi)$, which is the same as minimizing the regret $J_M(\pi_M^\star) - J_M(\pi)$ for a fixed $M$. However, their  equivalence in online RL relies on the fact that online exploration can eventually resolve any model uncertainty when needed, so we only need to consider the performance metrics w.r.t.~the true model $M=M^\star$. In offline RL with an arbitrary data distribution (i.e., we do not make any coverage assumptions), there will generally be model uncertainty that cannot be resolved, and worst-case reasoning over such model uncertainty (a.k.a.~the version space $\Mcal_\alpha$) separates apart the definitions that are once equivalent. 

Moreover, it is impossible to  compare  return maximization and regret minimization and make a claim about which one is better. They are not simply an algorithm design choice, but are definitions of the learning goals and the guarantees themselves---thus incomparable: if we care about obtaining a guarantee for the worst-case \textit{return}, then  return maximization is optimal by definition; if we are more interested in obtaining a guarantee for the worst-case \textit{regret}, then again, regret minimization is trivially optimal. We also note that analyzing algorithms under a metric that is different from the one they are designed for can lead to unusual conclusions. For example, \citet{xiao2021optimality} show that optimistic/neutral/pessimistic algorithms\footnote{Incidentally, optimistic/neutral policies  correspond to \#4 in Corollary~\ref{th:fixed-point examples}.} are equally minimax-optimal in terms of their regret guarantees in offline multi-armed bandits. However, the algorithms they consider are optimistic/pessimistic w.r.t.~the return---as commonly considered in the offline RL literature---not w.r.t.~the regret which is the performance metric they are interested in analyzing. 

\paragraph{$\piref$ is more than a hyperparameter---it defines the performance metric and learning goal} Corollary~\ref{th:fixed-point examples}  shows that \algo (with relative pessimism) has many different fixed points, some of which may seem quite unreasonable for offline learning, such as greedy w.r.t.~an arbitrary model or even optimism (\# 4). From the above discussion, we can see that this is not a defect of the algorithm. Rather, in the offline setting with unresolvable model uncertainty, there are many different performance metrics/learning goals that are generally incompatible/incomparable with each other, and the agent designer must make a choice among them and convey the choice to the algorithm. In \algo, such a choice is explicitly conveyed by the choice of $\piref$, which subsumes return maximization and regret minimization as special cases (\#2 and \#3 in Corollary~\ref{th:fixed-point examples}). 


%This result shows that fixed points of relative pessimism is not always sensible policies for offline RL, especially because $\pi_M^*$ is always a fixed point. 
%\textcolor{red}{In other words, designing $\psi(\cdot)$ can be viewed as one of the main design choices of offline RL based on version space.}
